Holistic Grid-Forming Control to Enhance the Frequency Support from HVDC-Connected Offshore Wind Power Plants

To address the frequency stability challenges posed by the rising penetration of power electronics in power systems, HVDC-connected offshore wind power plants (OWPPs) are increasingly expected to provide inertial response and frequency containment reserve (FCR). In this paper, an improved holistic grid-forming (GFM) control is proposed, aiming to enhance the frequency support by coordinating the GFM controls implemented at all AC and DC terminals of an HVDC-OWPP system, without requiring communication. Firstly, the model of a typical HVDC-OWPP system is developed for control design. Accordingly, the proposed controllers are formulated, followed by an analytical tuning method, where the upper bound of the bandwidth at each AC or DC terminal is identified. Finally, simulations are conducted to verify the functionality and compare the performance with that of representative control configurations. The results show that the proposed holistic GFM control achieves faster response and thus more effective frequency support, while the utilization of the inherent energy storage of each converter is minimized, thereby supporting a new design philosophy for converter control in converter-dominated systems.

==> Contents/Appx1.tex <==
% Use $\backslash${\tt{appendix}} if you have a single appendix:
% Do not use $\backslash${\tt{section}} anymore after $\backslash${\tt{appendix}}, only $\backslash${\tt{section*}}.
% If you have multiple appendixes use $\backslash${\tt{appendices}} then use $\backslash${\tt{section}} to start each appendix.
% You must declare a $\backslash${\tt{section}} before using any $\backslash${\tt{subsection}} or using $\backslash${\tt{label}} ($\backslash${\tt{appendices}} by itself
A general symmetrical three-phase AC transmission system is adopted, as shown in Fig. \ref{fig_URLE}, where the AC voltage source \textbf{\textit{u}} has phase-to-ground amplitude $U$ (V) and phase angle $\theta_{\text{u}}$ (rad); the AC voltage source \textbf{\textit{e}} has phase-to-ground amplitude $E$ (V) and phase angle $\theta_{\text{e}}$ (rad); $R$ ($\Omega$) and $L$ (H) are the resistance and inductance of the transmission line; \textbf{\textit{i}} is the transmission current with amplitude $I$ (A) and power factor angle $\phi$ (rad).
\begin{figure}[!t]
\centering
\includegraphics{Figures/URLE.pdf}
\caption{A general symmetrical three-phase AC power transmission system}
\label{fig_URLE}
\end{figure}

% \subsection{Nonlinear Model}
% \label{NonlinearPwr}
% According to KVL, the voltage balance of the system can be described as \eqref{ACKVL}.
% \begin{equation}
% \label{ACKVL}
% L \frac {\text{d}i^{j}} {\text{d}t} 
% = 
% u^{j}
% - e^{j} 
% - R i^{j}, 
% j \in {\{\text{a, b, c}\}}
% \end{equation}
% By applying the transformation defined by the matrix $\textbf{\textit{P}}$ in \eqref{ParkTrans} which implements a constant-amplitude Park-transformation with the d-axis aligned to \textbf{\textit{u}}, \eqref{ACKVL} can be transformed into \eqref{ACKVLdq0}, where $\delta$ (rad) is the power angle, and $\delta = \theta_{\text{u}} - \theta_{\text{e}}$; $\omega$ (rad/s) is the angular frequency of the AC system, assumed to be the nominal constant, $\omega_{\text{N}}$; $u^{\text{d}} = U$, and $u^{\text{q}} = 0$.
% \begin{equation}
% \label{ParkTrans}
% \textbf{\textit{P}} = \frac{2}{3}
% \begin{bmatrix} 
% \sin{(\theta_{\text{u}})} & \sin{(\theta_{\text{u}} - \frac{2\pi}{3})} & \sin{(\theta_{\text{u}} + \frac{2\pi}{3})} \\
% \cos{(\theta_{\text{u}})} & \cos{(\theta_{\text{u}} - \frac{2\pi}{3})} & \cos{(\theta_{\text{u}} + \frac{2\pi}{3})} \\
% \frac{1}{2}&\frac{1}{2} & \frac{1}{2}
% \end{bmatrix}
% \end{equation}
% \begin{equation}
% \label{ACKVLdq0}
% \begin{cases}
% L \frac {\text{d}i^{\text{d}}} {\text{d}t} 
% = 
% u^{\text{d}}
% - E\cos{\delta}
% - R i^{\text{d}}
% + \omega Li^{\text{q}}
% \\
% L \frac {\text{d}i^{\text{q}}} {\text{d}t} 
% = 
% u^{\text{q}}
% + E\sin{\delta}
% - R i^{\text{q}}
% - \omega Li^{\text{d}}
% \end{cases}
% \end{equation}
% By solving \eqref{ACKVLdq0}, $i^{\text{d,q}}$ can be expressed as \eqref{ACidq}, where "$s$" is the Laplace operator.
% \begin{equation}
% \label{ACidq}
%     \begin{cases}
%         i^{\text{d}} = \frac{ \omega  L E \sin \! \left(\delta \right)  + \left(L s +R \right) \left(U- E \cos \! \left(\delta \right) \right) }{(sL+R)^2+( \omega L)^2}
%         \\
%         i^{\text{q}} = \frac{ \omega  L \left(E \cos \! \left(\delta \right)-U \right) + \left(L s +R \right) E \sin \! \left(\delta \right)}{(sL+R)^2+( \omega L)^2}
%     \end{cases}
% \end{equation}
% Therefore, the active power output of source \textbf{\textit{u}} can be expressed as \eqref{NonLinPwr}.
% \begin{equation}
% \label{NonLinPwr}
% \begin{split}
%     P_{\text{u}}
%     &= \frac{3}{2}\left(u^{\text{d}}i^{\text{d}}+u^{\text{q}}i^{\text{q}}\right)
%     \\
%     &= \frac{3 U \left(  \omega  L E \sin \! \left(\delta \right)  + \left(L s +R \right) \left(U- E \cos \! \left(\delta \right) \right) \right) }{2\left((sL+R)^2+( \omega L)^2\right)}
% \end{split}
% \end{equation}

% \subsection{Linear Model with Virtual Resistance}
% \label{LinearPwr}
% Assuming constant voltage amplitudes, $U$ and $E$, by adding virtual resistance to \eqref{ACKVLdq0} and then linearizing it, the new voltage balance is obtained as \eqref{ACKVLdq0Linear}, where the subscript "o" denotes the initial operating point; $\Delta$ denotes the deviation from the initial operating point; $R_{\text{v}}$ ($\Omega$) and $T_{\text{v}}$ (s) are the virtual resistance and the corresponding time constant.
% \begin{equation}
% \label{ACKVLdq0Linear}
% \begin{cases}
% L s \Delta i^{\text{d}} 
% = 
% E_{\text{o}}\sin{\delta_{\text{o}}\Delta\delta}
% - R \Delta i^{\text{d}}
% +  \omega L\Delta i^{\text{q}}
% - \frac{R_{\text{v}}s}{s+1/T_{\text{v}}} \Delta i^{\text{d}}
% \\
% L s \Delta i^{\text{q}}
% = 
% E_{\text{o}}\cos{\delta_{\text{o}}\Delta\delta}
% - R \Delta i^{\text{q}}
% -  \omega L \Delta i^{\text{d}}
% - \frac{R_{\text{v}}s}{s+1/T_{\text{v}}} \Delta i^{\text{q}}
% \end{cases}
% \end{equation}
% By solving \eqref{ACKVLdq0Linear}, $\Delta i^{\text{d,q}}$ can be expressed by $\Delta \delta$ as \eqref{Deltaidq}. 
% \begin{align}
% \label{Deltaidq}
% &\begin{cases}
%     \Delta i^{\text{d}} = {\frac {E_{\text{o}}\, \left( T_{\text{v}}\,s+1 \right) 
%  \left( \alpha_{1} \cos \left( 
% \delta_{\text{o}} \right) + \alpha_{2} \sin
%  \left( \delta_{\text{o}} \right)  \right) }{ 
%  \beta_{4} s^4 + \beta_{3} s^3 + \beta_{2} s^2 + \beta_{1} s +\beta_{0}
%  }} \Delta \delta
% \\
% \Delta i^{\text{q}} = {\frac {E_{\text{o}}\, \left( T_{\text{v}}\,s+1 \right) \left(  \alpha_{2} \cos \left( \delta_{\text{o}} \right) -\alpha_{1} \sin \left( 
% \delta_{\text{o}} \right) \right) }{ 
%  \beta_{4} s^4 + \beta_{3} s^3 + \beta_{2} s^2 + \beta_{1} s + \beta_{0}}}\Delta \delta
% \end{cases} \\
% &\alpha_{1} =  \omega L \left( T_{\text{v}}\,s+1 \right), \alpha_{2} = LT_{\text{v}}s^2 + ((R+R_{\text{v}})T_{\text{v}}+L )s +R \notag \\
% &\beta_{4} = L^2T_{\text{v}}^2,  \beta_{3} = 2 L T_{\text{v}} \left(\left(R +R_{\text{v}} \right) T_{\text{v}} +L \right) \notag \\
% &\beta_{2} = \left(  \omega ^{2} L^{2} +\left(R +R_{\text{v}} \right)^{2}\right) T_{\text{v}}^{2}+4 L \left(R +\frac{R_{\text{v}}}{2}\right) T_{\text{v}} +L^{2} \notag \\
% &\beta_{1} = \left(2   \omega ^{2}L^{2}+2 R \left(R +R_{\text{v}} \right)\right) T_{\text{v}} +2 L R, \beta_{0} = \omega^2 L^2 + R^2 \notag
% \end{align}
% Thereupon, $\Delta u^{\text{d,q}}$ can be expressed by $\Delta \delta$ as \eqref{ACdeltaU}.
% \begin{equation}
% \label{ACdeltaU}
%     \begin{cases}
%     \Delta u^{\text{d}} = - \frac{R_{\text{v}}s}{s+1/T_{\text{v}}} \Delta i^{\text{d}} = -{\frac {R_{\text{v}} T_{\text{v}} E_{\text{o}} s \left( \alpha_{1} \cos \left( 
% \delta_{\text{o}} \right) + \alpha_{2} \sin
%  \left( \delta_{\text{o}} \right)  \right) }{ 
%  \beta_{4} s^4 + \beta_{3} s^3 + \beta_{2} s^2 + \beta_{1} s +\beta_{0}
%  }} \Delta \delta
%     \\
%     \Delta u^{\text{q}} = - \frac{R_{\text{v}}s}{s+1/T_{\text{v}}} \Delta i^{\text{q}} = - {\frac {R_{\text{v}} T_{\text{v}} E_{\text{o}} s \left(  \alpha_{2} \cos \left( \delta_{\text{o}} \right) -\alpha_{1} \sin \left( 
% \delta_{\text{o}} \right) \right) }{ 
%  \beta_{4} s^4 + \beta_{3} s^3 + \beta_{2} s^2 + \beta_{1} s + \beta_{0}}}\Delta \delta
%     \end{cases}
% \end{equation}
% Besides, the $u^{\text{d,q}}$ and $i^{\text{d,q}}$ at the initial operating point can be derived as \eqref{ACUoIo}, where $I_{\text{o}} = \frac{\sqrt{(u^{\text{d}}_{\text{o}}-E_{\text{o}}\cos{\delta_{\text{o}}})^2 + (u^{\text{q}}_{\text{o}} + E_{\text{o}}\sin{\delta_{\text{o}}})^2}}{\sqrt{R^2+( \omega L)^2}}$; $\phi_{\text{o}} = \arctan{(\frac{u^{\text{q}}_{\text{o}} + E_{\text{o}}\sin{\delta_{\text{o}}}}{u^{\text{d}}_{\text{o}} - E_{\text{o}}\cos{\delta_{\text{o}}}})} - \arctan{(\frac{ \omega L}{R}})$.
% \begin{equation}
% \label{ACUoIo}
%     \begin{cases}
%     u^{\text{d}}_{\text{o}} = U_{\text{o}} 
%     \\
%     u^{\text{q}}_{\text{o}} = 0
%     \end{cases}
%     \begin{cases}
%     i^{\text{d}}_{\text{o}} = I_{\text{o}}\cos{\phi_{\text{o}}} 
%     \\
%     i^{\text{q}}_{\text{o}} = I_{\text{o}}\sin{\phi_{\text{o}}}
%     \end{cases}
% \end{equation}
% By combining \eqref{Deltaidq}, \eqref{ACdeltaU}, and \eqref{ACUoIo}, the power response from \textbf{\textit{u}} can be expressed by $\Delta \delta$ as \eqref{PowerResponse}, where $G_{\text{Pac}}(s)$ denotes the transfer function from $\Delta \delta$ to $\Delta P_{\text{u}}$; $\varphi_{\text{o}}=\phi_{\text{o}}+\delta_{\text{o}}$.
% \begin{align}
% \label{PowerResponse}
%     &\Delta P_{\text{u}} = 
%     \frac{3}{2}
%     \left(
%     \begin{bmatrix}
%     u^{\text{d}}_{\text{o}} & u^{\text{q}}_{\text{o}}
%     \end{bmatrix} 
%     \begin{bmatrix}
%     \Delta i^{\text{d}} \\ \Delta i^{\text{q}}
%     \end{bmatrix}
%     +
%     \begin{bmatrix}
%     \Delta u^{\text{d}} & \Delta u^{\text{q}}
%     \end{bmatrix} 
%     \begin{bmatrix}
%     i^{\text{d}}_{\text{o}} \\ i^{\text{q}}_{\text{o}}
%     \end{bmatrix}
%     \right) \notag
%     \\
%     &= \underbrace{ \frac{3}{2} E_{\text{o}} \left( \frac{ \gamma_{3} s^3 + \gamma_{2} s^2 + \gamma_{1} s + \gamma_{0}}{ 
% \beta_{4} s^4 + \beta_{3} s^3 + \beta_{2} s^2 + \beta_{1} s + \beta_{0}} \right) }_{G_{\text{Pac}}(s)} \Delta \delta 
% \\
% &\gamma_{3}=L T_{\text{v}}^{2} \left(U_{\text{o}} \sin \! \left(\delta_{\text{o}} \right)-I_{\text{o}} R_{\text{v}} \sin \! \left(\phi_{\text{o}} +\delta_{\text{o}} \right)\right) \notag
% \\
% &\gamma_{2} = \left(U_{\text{o}} \left(\left(R +R_{\text{v}} \right) T_{\text{v}} +2 L \right) \sin \! \left(\delta_{\text{o}} \right)+L \cos \! \left(\delta_{\text{o}} \right) T_{\text{v}} U_{\text{o}}  \omega  \notag \\
% &-I_{\text{o}} \left(\left(R +R_{\text{v}} \right) T_{\text{v}} +L \right) R_{\text{v}} \sin \! \left(\varphi_{\text{o}} \right)-I_{\text{o}} L R_{\text{v}} T_{\text{v}}  \omega  \cos \! \left(\varphi_{\text{o}} \right)\right) T_{\text{v}} \notag
% \\
% &\gamma_{1} = U_{\text{o}} \left(\left(2 R +R_{\text{v}} \right) T_{\text{v}} +L \right) \sin \! \left(\delta_{\text{o}} \right)+2 L \cos \! \left(\delta_{\text{o}} \right) T_{\text{v}} U_{\text{o}}  \omega  \notag \\ 
% &-I_{\text{o}} R R_{\text{v}} T_{\text{v}} \sin \! \left(\varphi_{\text{o}} \right)-I_{\text{o}} L R_{\text{v}} T_{\text{v}}  \omega  \cos \! \left(\varphi_{\text{o}} \right) \notag
% \\
% &\gamma_{0} = U_{\text{o}} \left( \omega  L \cos \! \left(\delta_{\text{o}} \right)+\sin \! \left(\delta_{\text{o}} \right) R \right) \notag 
% \end{align}




==> Contents/Appx2.tex <==




% \subsection{Control Gains}

% \paragraph{Onshore \& Offshore MMC}
% $K_{\text{H,on}}$ (Hz/J): 1.5e-6; $K_{\text{H,off}}$ (Hz/J): 1.7e-6; $K_{\text{D,on}}$ (rad/Hz): 0.095; $K_{\text{D,off}}$ (rad/Hz): 0.097; $R_{\text{v,on}} (\Omega): 46$; $R_{\text{v,off}} (\Omega): 54$; $T_{\text{v,on}}$ (s): 0.021; $T_{\text{v,off}}$ (s): 0.018; $K_{\text{R,on}}$ (V/Hz): 38400; $K_{\text{R,off}}$ (V/Hz): 38400; $K_{\text{pUdc}}$ (A/V): 0.029; $K_{\text{iUdc}}$ (A/V): 5.8; $G_{\text{cmp}(s)} = \frac{3.5e^{-6}s^2+2.1e^{-4}s+16}{16(1e^{-4}s+1)^2}$; $K_{\text{pIdc}}$ (V/A): 130; $K_{\text{iIdc}}$ (V/A): 2048.

% \paragraph{OWPP}
% $K_{\text{Hlink}}$ (Hz/J): 1.0027; $K_{\text{Dlink}}$ (rad/Hz): 15.415; $R_{\text{vw}} (\Omega): 0.2512$; $T_{\text{vw}}$ (s): 0.0153.



==> Contents/RecycleBin.tex <==
By solving \eqref{ACKVLdq0Linear}, $\Delta i_{\text{d,q}}$ can be expressed by $\Delta \delta$ as \eqref{ACdeltai}.
\begin{equation}
\label{ACdeltai}
\left\{
\begin{array}{c}
\Delta i_{\text{d}}
= 
U_{\text{o}} \frac{\omega_{1}L\cos{\delta_{\text{o}}} - (sL+R)\sin{\delta_{\text{o}}}}{(sL+R)^2+(\omega_{1}L)^2} \Delta \delta
\\
\Delta i_{\text{q}}
= 
U_{\text{o}} \frac{\omega_{1}L\sin{\delta_{\text{o}}} + (sL+R)\cos{\delta_{\text{o}}}}{(sL+R)^2+(\omega_{1}L)^2} \Delta \delta
\end{array}
\right.
\end{equation}
Likewise, based on \eqref{ACKVLdq0}, $u_{\text{d,q}}$ can be linearized and expressed by $\Delta \delta$ as \eqref{ACdeltaU}.
\begin{equation}
\label{ACdeltaU}
    \begin{cases}
    \Delta u_{\text{d}} = -U_{\text{o}}\sin{\delta_{\text{o}}}\Delta \delta 
    \\
    \Delta u_{\text{q}} = U_{\text{o}}\cos{\delta_{\text{o}}}\Delta \delta
    \end{cases}
\end{equation}
Besides, the $u_{\text{d,q}}$ and $i_{\text{d,q}}$ at the initial operating point can be derived as \eqref{ACUo} and \eqref{ACIo}, where $I_{\text{o}} = \frac{\sqrt{(U_{\text{do}}-E_{\text{o}})^2 + U^2_{\text{qo}}}}{\sqrt{R^2+(\omega_{1}L)^2}}$; $\theta_{I\text{o}} = \arctan{(\frac{U_{\text{qo}}}{U_{\text{do}} - E_{\text{o}}})} - \arctan{(\frac{\omega_{1}L}{R}})$.
\begin{equation}
\label{ACUo}
    \begin{cases}
    u_{\text{do}} = U_{\text{o}}\cos{\delta_{\text{o}}} 
    \\
    u_{\text{qo}} = U_{\text{o}}\sin{\delta_{\text{o}}}
    \end{cases}
\end{equation}
\begin{equation}
\label{ACIo}
    \begin{cases}
    i_{\text{do}} = I_{\text{o}}\cos{\theta_{I\text{o}}} 
    \\
    i_{\text{qo}} = I_{\text{o}}\sin{\theta_{I\text{o}}}
    \end{cases}
\end{equation}
By combining \eqref{ACdeltai}, \eqref{ACdeltaU}, \eqref{ACUo}, and \eqref{ACIo}, the power response from \textbf{\textit{u}} can be expressed by $\Delta \delta$ as \eqref{PowerResponse}, where $\varphi_{\text{o}}$ (rad) is the inital power factor angle for source \textbf{\textit{u}}, and $\varphi_{\text{o}} = \theta_{I\text{o}} - \delta_{\text{o}}$.
\begin{equation}
\label{PowerResponse}
\begin{split}
    \Delta P_{\text{u}} &= \frac{3}{2}
    \left(
    \begin{bmatrix}
    u_{\text{do}} & u_{\text{qo}}
    \end{bmatrix} 
    \begin{bmatrix}
    \Delta i_{\text{d}} \\ \Delta i_{\text{q}}
    \end{bmatrix}
    +
    \begin{bmatrix}
    \Delta u_{\text{d}} & \Delta u_{\text{q}}
    \end{bmatrix} 
    \begin{bmatrix}
    i_{\text{do}} \\ i_{\text{qo}}
    \end{bmatrix}
    \right)
    \\
    &= \frac{3}{2}U_{\text{o}}
    \left(
    \frac{U_{\text{o}}\omega_{1}L}{(sL+R)^2+(\omega_{1}L)^2}
    + I_{\text{o}}\sin{(\varphi_{\text{o}})}
    \right) 
    \Delta \delta
\end{split}
\end{equation}

\subsection{Linear Model with Virtual Resistance}
\label{LinearPwr}
For better demonstration, per-unit value system is adopted for the electrical variables below without additional notation, with base values defined as \eqref{BaseValues}, where $U_{\text{b}}$ (V), $I_{\text{b}}$ (A), $Z_{\text{b}}$ ($\Omega$), $L_{\text{b}}$ (H), and $\omega_{\text{b}}$ (rad/s) are the base values for voltage, current, impedance, inductance, and angular frequency, respectively; $S_{\text{N}}$ (VA), $U_{\text{N}}$ (V), and $f_{\text{N}}$ (Hz) are the nominal capacity, voltage (line-to-line) and frequency.
\begin{equation}
\label{BaseValues}
    U_{\text{b}} = \sqrt{\frac{2}{3}}U_{\text{N}}, 
    I_{\text{b}} = \sqrt{\frac{2}{3}}\frac{S_{\text{N}}}{U_{\text{N}}},
    Z_{\text{b}} = \frac{U_{\text{b}}}{I_{\text{b}}},
    L_{\text{b}} = \frac{Z_{\text{b}}}{\omega_{\text{b}}},
    \omega_{\text{b}} = 2\pi f_{\text{N}}
\end{equation}
Assuming constant voltage amplitudes, $U$ and $E$, by neglecting $R$ ($R\ll$ L), adding virtual resistance to \eqref{ACKVLdq0} and then linearizing it, the new voltage balance is obtained as \eqref{ACKVLdq0Linear}, where the subscript "o" denotes the initial operating point; $\Delta$ denotes the deviation from the initial operating point; $R_{\text{v}}$ (p.u.) and $T_{\text{v}}$ (s) are the virtual resistance and the corresponding time constant.
\begin{equation}
\label{ACKVLdq0Linear}
\begin{cases}
\frac{L}{\omega_{\text{b}}} s \Delta i_{\text{d}} 
= 
- U_{\text{o}}\sin{\delta_{\text{o}}\Delta\delta}
- \frac{R_{\text{v}}s}{s+1/T_{\text{v}}} \Delta i_{\text{d}}
+ \omega_{1}L\Delta i_{\text{q}}
\\
\frac{L}{\omega_{\text{b}}} s \Delta i_{\text{q}}
= 
U_{\text{o}}\cos{\delta_{\text{o}}\Delta\delta}
- \frac{R_{\text{v}}s}{s+1/T_{\text{v}}} \Delta i_{\text{q}}
- \omega_{1}L \Delta i_{\text{d}}
\end{cases}
\end{equation}
By solving \eqref{ACKVLdq0Linear}, $\Delta i_{\text{d,q}}$ can be expressed by $\Delta \delta$ as \eqref{Deltaidq}, where $\alpha_{1} = L\omega_{1}\,\omega_{\text{b}}\, \left( T_{\text{v}}\,s+1 \right)$; $\alpha_{2} = s \left( sLT_{\text{v}}+R_{\text{v}}\,T_{\text{v}}\,\omega_{\text{b}}+L \right)$; $\beta = 1+ \frac{R_{\text{v}}T_{\text{v}}\omega_{\text{b}}-2L}{2L(T_{\text{v}}s+1)} - \frac{R_{\text{v}}T_{\text{v}}\omega_{\text{b}}}{2L(T_{\text{v}}s+1)^2}$. 
\begin{align}
\label{Deltaidq}
\begin{cases}
    \Delta i_{\text{d}} = {\frac {\omega_{\text{b}}\, U_{\text{o}}\, \left( T_{\text{v}}\,s+1 \right) 
 \left( \alpha_{1} \cos \left( 
\delta_{\text{o}} \right) - \alpha_{2} \sin
 \left( \delta_{\text{o}} \right)  \right) }{ 
 L^2 (T_{\text{v}}s+1)^2 ( s^2 +2 \beta \frac{R_{\text{v}}}{L}\omega_{\text{b}} s+\omega_{\text{1}}^2\omega_{\text{b}}^2 )
 }} \Delta \delta
\\
\Delta i_{\text{q}} = {\frac {\omega_{\text{b}}\, U_{\text{o}}\, \left( T_{\text{v}}\,s+1 \right) \left( \alpha_{1} \sin \left( 
\delta_{\text{o}} \right) + \alpha_{2} \cos \left( \delta_{\text{o}} \right) \right) }{ 
 L^2 (T_{\text{v}}s+1)^2 ( s^2 +2 \beta \frac{R_{\text{v}}}{L}\omega_{\text{b}} s+\omega_{\text{1}}^2\omega_{\text{b}}^2 )}}\Delta \delta
\end{cases}
\end{align}
Likewise, based on \eqref{ACKVLdq0}, $u_{\text{d,q}}$ can be linearized and expressed by $\Delta \delta$ as \eqref{ACdeltaU}.
\begin{equation}
\label{ACdeltaU}
    \begin{cases}
    \Delta u_{\text{d}} = -U_{\text{o}}\sin{\delta_{\text{o}}}\Delta \delta 
    \\
    \Delta u_{\text{q}} = U_{\text{o}}\cos{\delta_{\text{o}}}\Delta \delta
    \end{cases}
\end{equation}
Besides, the $u_{\text{d,q}}$ and $i_{\text{d,q}}$ at the initial operating point can be derived as \eqref{ACUoIo}, where $I_{\text{o}} = \frac{\sqrt{(U_{\text{do}}-E_{\text{o}})^2 + U^2_{\text{qo}}}}{\sqrt{R^2+(\omega_{1}L)^2}}$; $\theta_{I\text{o}} = \arctan{(\frac{U_{\text{qo}}}{U_{\text{do}} - E_{\text{o}}})} - \arctan{(\frac{\omega_{1}L}{R}})$.
\begin{equation}
\label{ACUoIo}
    \begin{cases}
    u_{\text{do}} = U_{\text{o}}\cos{\delta_{\text{o}}} 
    \\
    u_{\text{qo}} = U_{\text{o}}\sin{\delta_{\text{o}}}
    \end{cases}
    \begin{cases}
    i_{\text{do}} = I_{\text{o}}\cos{\theta_{I\text{o}}} 
    \\
    i_{\text{qo}} = I_{\text{o}}\sin{\theta_{I\text{o}}}
    \end{cases}
\end{equation}
By combining \eqref{Deltaidq}, \eqref{ACdeltaU}, and \eqref{ACUoIo}, the power response from \textbf{\textit{u}} can be expressed by $\Delta \delta$ as \eqref{PowerResponse}, where $\varphi_{\text{o}}$ (rad) is the inital power factor angle for source \textbf{\textit{u}}, and $\varphi_{\text{o}} = \theta_{I\text{o}} - \delta_{\text{o}}$.
\begin{equation}
\label{PowerResponse}
\begin{split}
    \Delta P_{\text{u}} &= 
    \begin{bmatrix}
    u_{\text{do}} & u_{\text{qo}}
    \end{bmatrix} 
    \begin{bmatrix}
    \Delta i_{\text{d}} \\ \Delta i_{\text{q}}
    \end{bmatrix}
    +
    \begin{bmatrix}
    \Delta u_{\text{d}} & \Delta u_{\text{q}}
    \end{bmatrix} 
    \begin{bmatrix}
    i_{\text{do}} \\ i_{\text{qo}}
    \end{bmatrix} \\
    &= \underbrace{ U_{\text{o}} \left( \frac{ \omega_{1} U_{\text{o}} \omega^2_{\text{b}} }{ 
 L ( s^2 +2 \beta \frac{R_{\text{v}}}{L}\omega_{\text{b}} s+\omega_{\text{1}}^2\omega_{\text{b}}^2 )} + I_{\text{o}} \sin{\varphi_{\text{o}}} \right) }_{G_{\text{Pac}}(s)} \Delta \delta
\end{split}
\end{equation}


\subsection{Virtual Resistance Tuning}

\subsubsection{Location of Poles}
With $\omega_{1}$ (p.u.) maintained closely around 1, the two poles of $G_{\text{Pac}}(s)$ in \eqref{PowerResponse} have the natural frequency of $\omega_{\text{b}}$ (rad/s) and damping ratio defined by $\beta \frac{R_{\text{v}}}{L}$, where the range of $\beta$ is bounded by the limit in \eqref{BetaLimit}.

\begin{equation}
\label{BetaLimit}
    \lim_{T_{\text{v}} \to T_{\text{lmt}}} \beta(|s|=\omega_{\text{b}}) = 
    \begin{cases}
        0, &T_{\text{lmt}} = 0 \\
        1+\frac{R_{\text{v}}}{2L}, &T_{\text{lmt}} = +\infty
    \end{cases}
\end{equation}
Therefore, $T_{\text{v}}$, $R_{\text{v}}$, and $L$ together determine the damping ratio of $G_{\text{Pac}}(s)$

\subsubsection{Location of Zeros}
